A Binary Optimization Approach for Constrained K-Means Clustering

K-Means clustering still plays an important role in many computer vision problems. While the conventional Lloyd method, which alternates between centroid update and cluster assignment, is primarily used in practice, it may converge to a solution with empty clusters. Furthermore, some applications may require the clusters to satisfy a specific set of constraints, e.g., cluster sizes, must-link/cannot-link. Several methods have been introduced to solve constrained K-Means clustering. Due to the non-convex nature of K-Means, however, existing approaches may result in sub-optimal solutions that poorly approximate the true clusters. In this work, we provide a new perspective to tackle this problem. Particularly, we reconsider constrained K-Means as a Binary Optimization Problem and propose a novel optimization scheme to search for feasible solutions in the binary domain. This approach allows us to solve constrained K-Means where multiple types of constraints can be simultaneously enforced. Experimental results on synthetic and real datasets show that our method provides better clustering accuracy with faster runtime compared to several commonly used techniques.

==> tex/dummy.tex <==
The algorithm proposed in our work is inspired by recent works on binary optimization~\cite{yuan2017exact}. Before proceeding, we first reformulate~\eqref{eq:S_udpate} as a binary optimization problem in the $\{-1,1\}$ domain. Specifically, let $\bP = 2\bS - \bOnes$ ($\bOnes$ is the matrix with all ones that has the same size as $\bS$), $\bD = \frac{1}{2}\bY$, the problem~\eqref{eq:S_udpate} can be written equivalently as
\begin{subequations}
    \label{eq:S_udpate_P}
    \begin{align}
    & \min_{\bP}  && \langle \bD, \bP \rangle, \\
    & \text{subject to} && \bP_{ij} \in \{-1, 1\}, \\
    & && \sum_{i=1}^k \bP_{ij} = 2 - k \;\; \forall j = 1\dots N, \\
    & && 2l_i - N \le \sum_{j=1}^N \bP_{ij} \le 2u_i - N \;\; \forall i=1 \dots k.\\
    & && \bP_{ip} = \bP_{iq}, \;\; i = 1\dots k \;\; \forall (\bx_p, \bx_q) \in \cM_t, \; t=1\dots m. \label{eq:S_udpate_P:must_link} \\
    & && \bP_{ip} + \bP_{iq} \le 1, \;\; i = 1\dots k \;\; \forall (\bx_p, \bx_q) \in \cD_t, \; t=1\dots m. \label{eq:S_udpate_P:must_not_link}
    \end{align}
\end{subequations}
Note that since $\bS \in \{0, 1\}$, $\bP = 2\bS - \bOnes \in \{-1,1\}$. With such change of variables,~\eqref{eq:S_udpate_linear} and~\eqref{eq:S_udpate_P} are equivalent. 

Furthermore, by introducing $\bQ \in \bbR^{k\times N}$ as an auxiliary, it can be proven (see supplementary material) that~\eqref{eq:S_udpate_P} is equivalent to
\begin{subequations}
    \label{eq:S_udpate_PQ}
    \begin{align}
    & \min_{\bP, \bQ}  && \langle \bD, \bP \rangle, \\ 
    & \text{subject to} && -1 \le \bP_{ij} \le 1  \\
    & && \sum_{i=1}^k \bP_{ij} = 2 - k \;\; \forall j = 1\dots N, \\
    & && 2l_i - N \le \sum_{j=1}^N \bP_{ij} \le 2u_i - N \;\; \forall i=1 \dots k. \\
    & && \bP_{ip} = \bP_{iq}, \;\; i = 1\dots k \;\; \forall (\bx_p, \bx_q) \in \cM_t, \; t=1\dots m. \label{eq:S_udpate_PQ:must_link} \\
    & && \bP_{ip} + \bP_{iq} \le 1, \;\; i = 1\dots k \;\; \forall (\bx_p, \bx_q) \in \cD_t, \; t=1\dots m. \label{eq:S_udpate_PQ:must_not_link}\\
    & && \langle \bP, \bQ \rangle = Nk, \|\bQ\|^2_F \le Nk
    \end{align}
\end{subequations}
By the introduction of $\bQ$, the binary problem~\eqref{eq:S_udpate_P} is converted into an equivalent optimization problem over the continuous domain~\eqref{eq:S_udpate_PQ}. However, due to the bi-linear constraint $\langle \bP, \bQ \rangle = Nk$,~\eqref{eq:S_udpate_PQ} is still non-convex and solving it globally is by no mean an easy task. To optimize~\eqref{eq:S_udpate_PQ}, inspired by the method proposed in~\cite{yuan2017exact}, we proposed to solve the following penalty problem:
\begin{subequations}
    \label{eq:S_udpate_PQ_penalty}
    \begin{align}
    & \min_{\bP, \bQ}  && \langle \bD, \bP \rangle + \rho(Nk - \langle \bP, \bQ \rangle ) \\ 
    & \text{subject to} && -1 \le \bP_{ij} \le 1  \\
    & && \sum_{i=1}^k \bP_{ij} = 2 - k \;\; \forall j = 1\dots N, \\
    & && 2l_i - N \le \sum_{j=1}^N \bP_{ij} \le 2u_i - N \;\; \forall i=1 \dots k. \\
    & && \bP_{ip} = \bP_{iq}, \;\; i = 1\dots k \;\; \forall (\bx_p, \bx_q) \in \cM_t, \; t=1\dots m. \label{eq:S_udpate_PQ_penalty:must_link} \\
    & && \bP_{ip} + \bP_{iq} \le 1, \;\; i = 1\dots k \;\; \forall (\bx_p, \bx_q) \in \cD_t, \; t=1\dots m. \label{eq:S_udpate_PQ_penalty:must_not_link}\\
    & && \|\bQ\|^2_F \le Nk
    \end{align}
\end{subequations}
where $\rho$ is the penalty parameter. 

Observe that~\eqref{eq:S_udpate_PQ_penalty} can be tackled by updating  $\bP$ and $\bQ$ alternatively. In such alternating scheme, the update steps for $\bP$ and $\bQ$ are convex, which can be solved efficiently using any off-the-shelf solvers. In fact, the optimal solution in the $\bQ$ update step can be computed in closed form. Specifically, the update steps for $\bP$ and $\bQ$ are as follows
\subsubsection{$\bP$ update}
With the matrix $\bQ$ fixed, updating $\bP$ amounts to solving a convex Linear Programming problem
\begin{subequations}
    \label{eq:S_udpate_P_update}
    \begin{align}
    & \min_{\bP}  && \langle \bD - \rho \bQ, \bP \rangle \\ 
    & \text{subject to} && -1 \le \bP_{ij} \le 1  \\
    & && \sum_{i=1}^k \bP_{ij} = 2 - k \;\; \forall j = 1\dots N, \\
    & && 2l_i - N \le \sum_{j=1}^N \bP_{ij} \le 2u_i - N \;\; \forall i=1 \dots k. \\
    & && \bP_{ip} = \bP_{iq}, \;\; i = 1\dots k \;\; \forall (\bx_p, \bx_q) \in \cM_t, \; t=1\dots m. \label{eq:S_udpate_P_update:must_link} \\
    & && \bP_{ip} + \bP_{iq} \le 1, \;\; i = 1\dots k \;\; \forall (\bx_p, \bx_q) \in \cD_t, \; t=1\dots m. \label{eq:S_udpate_P_update:must_not_link}\\
    \end{align}
\end{subequations}
\subsubsection{$\bQ$ update}
The update step of $\bQ$ with a fixed $\bP$ can be done by solving the following problem
\begin{subequations}
    \label{eq:S_udpate_Q_update}
    \begin{align}
    & \min_{\bQ}  &&  - \langle \bP, \bQ \rangle \\ 
    & \text{subject to} && \|\bQ\|^2_F \le Nk       
    \end{align}
\end{subequations}
In fact,~\eqref{eq:S_udpate_Q_update} can be updated by the following closed-form formular:
\begin{equation}
    \label{eq:S_udpate_Q_update_closed_form}
    \bQ = \begin{cases}
    \frac{\sqrt[]{Nk}}{\|\bP\|_F}\bP, \;\;\; \bP \neq \mathbf{0}_{N \times k } \\
    \mathbf{0}_{N\times k}, \;\;\; \text{otherwise.}
    \end{cases}
\end{equation}
